Classifying Trusted Hardware via Unidirectional Communication

It is well known that Byzantine fault tolerant (BFT) consensus cannot be solved in the classic asynchronous message passing model when one-third or more of the processes may be faulty. Since many modern applications require higher fault tolerance, this bound has been circumvented by introducing non-equivocation mechanisms that prevent Byzantine processes from sending conflicting messages to other processes. The use of trusted hardware is a way to implement non-equivocation. Several different trusted hardware modules have been considered in the literature. In this paper, we study whether all trusted hardware modules are equivalent in the power that they provide to a system. We show that while they do all prevent equivocation, we can partition trusted hardware modules into two different power classes; those that employ shared memory primitives, and those that do not. We separate these classes using a new notion we call unidirectionality, which describes a useful guarantee on the ability of processes to prevent network partitions. We show that shared-memory based hardware primitives provide unidirectionality, while others do not.

==> prelims.tex <==

\section{Old stuff}

We define three categories of communication depending on how much \correct{} processes hear from each other.

\begin{definition}[Bidirectional communication]
	A system provides \emph{bidirectional communication} if it can implement \emph{rounds} with the following property:
	
	For any pair of correct processes $p$ and $q$, if $p$ sends a message to $q$ in round $r$, then  $q$ receives round $r$ message from $p$ before the beginning $q$'s round $r+1$.
\end{definition}

\begin{definition}[Unidirectional communication]
	A system provides \emph{unidirectional communication} if it can implement \emph{rounds} with the following property:
	
	For any pair of correct processes $p$ and $q$, if both $p$ and $q$ send a message to each other in round $r$, then either $p$ receives $q$'s message before the beginning of $p$'s next round or $q$ receives $p$'s message before the beginning of $q$'s next round.
\end{definition}

\begin{definition}[Zero-directional communication]
	A system provides \emph{zero-directional communication} if it can implement \emph{rounds} with the following property:
	
	For a given pair of correct processes $p$ and $q$, if both $p$ and $q$ send a message to each other in round $r$, then it is possible that neither processes receive messages from the other processes before beginning their next round.
\end{definition}

\subsection{Relationship to Classical Communication Models}

\subsubsection{Communication Models Providing Only Zero-directionality}
\paragraph{Asynchronous communication.}
We note that the classic asynchronous model cannot guarantee more than zero-directional communication; while we can implement rounds in which $n-f$ messages are received by every correct process, we cannot guarantee successful communication between any given pair of processes.

\subsubsection{Communication Models Providing Bidirectionality}

\paragraph{Lock-step synchronous communication.}
The classic synchronous (lock-step) model requires the execution to be partitioned into rounds and in each round such that a message sent by a correct process $p$ to a correct process $q$ in one round arrives at process $q$ by the end of its round. This is exactly the same guarantee as bidirectional communication. Typically, lock-step synchronous communication can be realized using $\Delta$-synchronous communication using clock synchronization protocols as described in \cite{dolev1995dynamic, abraham2019sync}. Each round can be realized in $2\Delta$ time. %in each round; all messages sent by correct processes in a given round arrive at correct processes in the same round, as is the case with bidirectional communication.

\paragraph{$\Delta$-synchronous communication with synchronized clocks.}
gives us bidirectionality \kartik{will dig more}

\subsubsection{Communication Models Providing Unidirectionality}
\paragraph{$\Delta$-synchronous communication.} In the $\Delta$-synchronous model, there is a pessimistic upper bound $\Delta$ on the amount of time a message takes to arrive from the time at which it is sent. This bound may be much larger than the actual time, $\delta$, that a message takes. Note that in this model, waiting less than $\Delta$ time cannot ensure anything stronger than zero-directional communication, and waiting less than $2\Delta$ only ensures unidirectional communication. \kartik{will prove}

\paragraph{Asynchronous communication with shared-memory registers.}
Consider a shared memory setting with a single-writer multi-reader (SWMR) register per process. We now show that the communication achievable in this setting is \emph{unidirectional}.

\kartik{trusted processes + non-equivocation: relationship to unidirectionality; mapping between trusted processes $<->$ non-equivocation.}

\begin{claim}
	SWMR registers can implement  unidirectional communication.
\end{claim}
\begin{proof}
	We present an implementation of a unidirectional round in the SWMR register setting. This protocol was first introduced in~\cite{aguilera2019impact} to implement a weak notion of broadcast.
	
	\begin{lstlisting}
	In round r, process p executes the following:
	To send message m, p writes (r,m) in its register
	p reads the registers of all other processes
	p is said to receive a round r message m' from process q if p read (r,m') in q's register
	\end{lstlisting}
	
	Assume by contradiction that the above implementation of rounds does not satisfy unidirectionality. That is, there exist two correct processes $p$ and $q$ that both send a message in round $r$, but neither receive the other's message. Assume without loss of generality that $p$ wrote its round $r$ message in its register before $q$ did so in its own register. Then, since $q$ must write its message before reading $p$'s register, $q$ must see $p$'s round r message when it reads its register. Contradiction.
\end{proof}

\begin{claim}
	Anything that can be solved using asynchronous SWMR registers can also be solved using unidirectional communication.
\end{claim}

\begin{proof}[Proof sketch; to be filled out.]
	Argue about executions; if something happens in the unidirectional execution, show how the same thing can happen in the execution with registers.
\end{proof}


\paragraph{Asynchronous communication with sticky bits.}

% \paragraph{Asynchronous communication }




\section{Problems Considered}
We consider several problems and evaluate how much communication is required to solve them with various levels of fault tolerance.

\subsection{Broadcast}

%\subsection{Broadcast}
We consider three variants of broadcast, which differ in their termination requirements. We present them in order from weakest to strongest.

\Naama{Similar to crusader agreement.}
\begin{definition}[Non-Equivocating Broadcast]
In a non-equivocating broadcast protocol, a designated process $p_1$ receives an input value $v$, and acts as the \emph{sender}. The following conditions must be satisfied.
\begin{itemize}
    \item \textbf{Agreement. } If two \correct{} processes commit values $b$ and $b'$ respectively, then $b = b'$.
    %or $b = \bot$ or $b' = \bot$ where $\bot$ is a special value that cannot be sent by any process.
    \item \textbf{Validity/Termination.} If the sender is \correct{}, all \correct{} processes eventually commit the value $v$.
    %\item \textbf{Validity.} If the sender is \correct{}, then all \correct{} processes commit the value $v$.
\end{itemize}
\end{definition}
%\kartik{are termination and agreement at odds here since a process can commit a $\bot$}

\begin{definition}[Reliable Broadcast]
In a reliable broadcast protocol, a designated process $p_1$ receives an input value $v$, and acts as the \emph{sender}. The following three conditions must be satisfied.
\begin{itemize}
    \item \textbf{Agreement. } If two \correct{} processes commit values $b$ and $b'$ respectively, then $b = b'$.
    \item \textbf{Termination.} If a \correct{} process commits a value, then eventually all \correct{} processes commit a value.
    \item  \textbf{Validity.} If the sender is \correct{}, then all \correct{} processes commit the value $v$.
\end{itemize}
\end{definition}

\begin{definition}[Byzantine Broadcast]
In a Byzantine broadcast protocol, a designated process $p_1$ receives an input value $v$, and acts as the \emph{sender}. The following three conditions must be satisfied.
\begin{itemize}
    \item \textbf{Agreement. } If two \correct{} processes commit values $b$ and $b'$ respectively, then $b = b'$.
    \item \textbf{Termination.} All \correct{} processes eventually commit a value.
    \item \textbf{Validity.} If the sender is \correct{}, then all \correct{} processes commit the value $v$.
\end{itemize}
\end{definition}

\subsection{Agreement}

\begin{definition}[Very Weak Agreement]
In very weak validity agreement, each process receives an input value. The protocol must satisfy the following conditions:
\begin{itemize}
    \item \textbf{Agreement.} If two \correct{} processes commit values $v$ and $v'$, then either $v = v'$ or $v = \bot$ or $v' = \bot$.
    \item \textbf{Termination.} All \correct{} processes must eventually commit a value.
    \item \textbf{Weak Validity.} If all processes are \correct{} and they all received the same input $v$, then all processes commit $v$.
\end{itemize}
\end{definition}

\begin{definition}[Weak Validity Agreement]
In weak validity agreement, each process receives an input value. The protocol must satisfy the following conditions:
\begin{itemize}
    \item \textbf{Agreement.} If two \correct{} processes commit values $v$ and $v'$, then $v = v'$.
    \item \textbf{Termination.} All \correct{} processes must eventually commit a value.
    \item \textbf{Weak Validity.} If all processes are \correct{} and they all received the same input $v$, then all processes commit $v$.
\end{itemize}
\end{definition}

\begin{definition}[Strong Validity Agreement]
In strong validity agreement, each process receives an input value. The protocol must satisfy the following conditions:
\begin{itemize}
    \item \textbf{Agreement.} If two \correct{} processes commit values $v$ and $v'$, then $v = v'$.
    \item \textbf{Termination.} All \correct{} processes must eventually commit a value.
    \item \textbf{Strong Validity.} If all \correct{} processes received the same input $v$, then all \correct{} processes commit $v$.
\end{itemize}
\end{definition}



==> separations.tex <==
\section{Separation Results}




\subsection{Separating Bidirectional Communication from Unidirectional Communication}


\ignore{
\begin{claim}
Unidirectional communication cannot solve Byzantine broadcast with $n\leq 3f$.https://www.overleaf.com/project/5e8f94681d9c8a00012eba5d
\end{claim}

\begin{proof}[Proof Sketch.]
Assume by contradiction that we can implement Byzantine broadcast in a system with unidirectional communication and $n\leq 3f$. Then consider the following algorithm for strong Byzantine agreement:
\begin{itemize}
    \item Each process broadcasts its input value to all other processes.
    \item Each process waits to deliver a value from all processes, and commits the majority value of those it delivered. \Naama{Are Byzantine processes allowed not to broadcast at all? If so, this proof doesn't go through}
\end{itemize}
Then a majority of the values that each process delivered from the broadcast come from \correct{} processes and must be the same. Therefore, all \correct{} processes commit the same value, and that value was the input of some \correct{} process.
\end{proof}
}

\begin{claim}\label{clm:unidirSBA}
Strong validity agreement cannot be solved with unidirectionality in a system with $n\leq 3f$.
\end{claim}

\begin{proof}[Rough Sketch]
We proved that read/write registers can't solve strong validity agreement with $n \leq 3f$. This result also appeared in a slightly different form in \cite{malkhi2003objects}.
\end{proof}

\Naama{We know from classic results that bidirectional communication can solve strong validity agreement with $n\geq 2f+1$ with signatures. --- With Claim~\ref{clm:unidirSBA} this gives a separation between bidirectional and unidirectional communication.}


\begin{claim}\label{clm:wva-no-uni}
Weak validity agreement cannot be solved with unidirectional communication for $f \geq n/2$.
\end{claim}

\begin{proof}
Assume by contradiction that there exists an algorithm $A$ that can solve weak validity agreement in a system where $n = 2f$ with unidirectional communication. 
Consider four sets of processes, $P$, $Q$, $R$ and $S$. Assume $|P| = n-f-1$, $|Q| = 1$, $|R| = n-f-1$, and $|S| = 1$. Observe that $|P| = |R| = n-f-1 < f$.

% Assume that all processes in $P$ receive input $0$, and all processes in $R$ receive input $1$. 
Consider the following scenarios.
\paragraph{World~1.} All processes are correct, and all processes receive input $0$. All processes in $P$ receive messages from each other, and from $Q$, but do not receive messages from any other process for arbitrarily long. Processes in $R$ and $S$ receive messages from all parties. Since all processes are correct, validity and termination properties hold. Hence, all processes (and in particular, processes in $P$) commit $0$.

\paragraph{World~2.} All processes are correct and receive input $1$. All processes in $R$ hear from each other and from $Q$, but do not hear from any other process for arbitrarily long. Processes in $P$ and $S$ receive messages from all other processes. Since all processes are correct, validity and termination properties hold. Hence, all processes (and in particular, processes in $R$) commit $1$.

\paragraph{World~3.} Processes $Q$ and $R$ are Byzantine. Processes in $P$ and $S$ receive input $0$. $Q$ pretends to have input $0$ when communicating with $P$, and pretends to have input $1$ when communicating with $R$. $R$ sends messages to $S$ pretending to be correct and have input $1$, but not to hear any of $P$'s messages. $P$ does not receive any messages from $R$ or $S$ for arbitrarily long. $S$ receives all messages. Then this world is indistinguishable to $P$ from World~1, so processes in $P$ must commit $0$. Since $S$ is correct, it must also commit $0$.

\paragraph{World~4.} $Q$ and $P$ are Byzantine. $Q$ pretends to have input $0$ when communicating with $P$, and pretends to have  input $1$ when communicating with $R$. $P$ send messages to $S$ pretending to be correct and have input $0$, but not to hear any of $R$'s messages. $R$ does not receive any messages from $P$ or $S$ for arbitrarily long. $S$ receives all messages. Then this world is indistinguishable to $R$ from World~2, so processes in $R$ must commit $1$. Since $S$ is correct, it must also commit $1$. However, this world is indistinguishable to $S$ from World~3.



\noindent
\textbf{Scenario 1.} All processes in $Q$ and $R$ are \correct, and those in $P$ are Byzantine. In the execution, the processes in $R$ only receive messages from each other, and not from any process in $P$ or $Q$. Furthermore, processes in $P$ send messages as if they are \correct{} processes with input $0$ but are only receiving messages from each other. $Q$ receives all messages from both $R$ and $P$. Then, by the validity and termination conditions of weak validity agreement, eventually the processes in $R$ must terminate and commit $1$. Furthermore, by agreement, since the processes in $R$ commit $1$, $Q$ must eventually commit $1$ as well.

\noindent
\textbf{Scenario 2.} All processes in $Q$ and $P$ are \correct, and those in $R$ are Byzantine. In the execution, the processes in $P$ only receive messages from each other, and not from any process in $R$ or $Q$. 
Furthermore, processes in $R$ send exactly the same message as they would have in scenario 1. $Q$ receives all messages from both $P$ and $R$.
Then, by the validity and termination conditions of weak validity agreement, eventually the processes in $P$ must terminate and commit $0$. Furthermore, by agreement, since the processes in $P$ commit $0$, $Q$ must eventually commit $1$ as well. However, this scenario is indistinguishable to $Q$ from scenario 1, in which it must commit to a different value. Contradiction.

\Naama{Slight subtlety: can the correct processes not hearing from anyone else deduce that they can commit $\bot$? Not within any bounded amount of time...}
\end{proof}

\Naama{Using Dolev-Strong, we know that Byzantine broadcast can be solved with bidirectional communication with $n\geq f+1$. To solve weak agreement, choose some designated sender and have them broadcast their value to everyone. Commit the value delivered from the broadcast. ---- So with Claim~\ref{clm:wva-no-uni} we have a separation between bidirectional and unidirectional.}

\begin{claim}
Given bidirectional communication we can implement  unidirectional communication.
\end{claim}

\begin{proof}
Follows directly from the definition.
\end{proof}


\subsection{Separating Unidirectional Communication from Zero-Directional Communication}
\ignore{
\begin{claim}
Unidirectional communication can solve reliable broadcast with $n\geq 2f+1$.
\end{claim}

\begin{proof}
Aguilera et al.~\cite{aguilera2019impact} present an algorithm that solves reliable broadcast with SWMR registers in a system with $n\geq 2f+1$ processes. \Naama{The cleanest way to complete this to unidirecitonality is to separately show that unidirectionality can do everything the SWMR model can do.}
\end{proof}
}

\begin{claim}
Weak validity agreement can be solved with unidirectional communication for $n \geq 2f+1$.
\end{claim}

\begin{proof}[Rough Sketch]
Aguilera et al~\cite{aguilera2019impact} solve weak validity agreement with $n > 2f$ using read/write registers. Should be able to rewrite result to use unidirectional communication. \Naama{Again, to complete this to a proof for unidirectionality, need to show unidir can implement SWMR registers.}
\end{proof}

\Naama{Classic results show that zero-directional communication (asynchrony) needs $n\geq 3f+1$ to solve weak validity agreement (DLS).}

\begin{claim}
Given unidirectional communication we can implement zero-directional communication.
\end{claim}

\begin{proof}
Follows directly from the definition.
\end{proof}

\subsection{Comparing Unidirectional Communication and Non-Equivocation}

% Honest majority
% Unidirectionality can solve reliable broadcast: proven in Naama's paper but need to convert to unidirectionality
% Non-equivocating broadcast cannot solve unidirectionality: done: claim 4.6
% We do not know of an interesting problem that can be solved using unidirectionality

% Dishonest majority setting
% Reliable broadcast cannot solve unidirectionality: claim 4.6
% Unidirectionality cannot solve reliable broadcast --> to prove, 4.13
% Unidirectionality can solve and reliable broadcast cannot solve very weak agreement under dishonest majority, claim 4.11, 4.12
% Reliable broadcast can solve blah under dishonest majority --> to prove




\Naama{Non-equivocation is reliable broadcast.}

% \subsubsection{Honest Majority}

We now show that reliable broadcast is strictly weaker than unidirectionality except in some corner cases. Intuitively, the result holds because of the inability of reliable broadcast to break through a network partition between two \correct{} processes. This result therefore holds even for stronger variants of non-equivocation, as long as the only guarantee they give is \emph{eventual} delivery.

\begin{claim}
Reliable broadcast cannot implement unidirectionality in a system with $n > f+2$ and $f>1$, under asynchrony and in the absence of additional assumptions.
\end{claim}

\begin{proof}
Assume by contradiction that there exists a protocol $P$ that uses reliable broadcast and implements a unidirectional round in a system with $n > f+2$ and $f>1$. Partition the processes into three sets, $Q$, $C_1$, and $C_2$, where $|Q| = n-f$, $|C_1| = 1$, and $|C_2| = f-1$. 
Consider the following scenarios.

\paragraph{Scenario~1.} The process $p \in C_1$ is faulty, and all the others are \correct. $p$ crashes at the beginning of the execution and never sends any messages, and all messages from $C_2$ to processes in $Q$ are arbitrarily delayed. All other messages are received immediately. Then processes in $Q$ must eventually start the next round since, from the perspective of $Q$, $C_1$ and $C_2$ could both have been faulty, in which case the number of faults is $\leq f$. This satisfies the problem constraint. Similarly, $C_2$ must eventually start the next round, since they are receiving all messages sent by correct processes, which are $> n-f$. 

Observe that in this scenario, a process in $C_2$ starts the next round without receiving a message from $C_1$.
%Then processes in $C_2$ output a vector in which slot $p$ does not contain $v_p$, since they cannot know its input.

\paragraph{Scenario~2.} The processes in $C_2$ are faulty, and the rest are \correct. No process in $C_2$ sends any messages, and all messages from $C_1$ to $Q$ are arbitrarily delayed. All other messages are received immediately. Using the same reasoning as in Scenario~1, processes in $Q$ and $C_1$ must eventually start the next round.
%, and the process in $C_1$ must eventually terminate this round and start the next one, since it is receiving all messages sent by correct processes. 

Observe that in this scenario, a process in $C_1$ starts the next round without receiving a message from any party in $C_2$. %Then clearly, $p$ does not receive any messages from $C_2$ in this round.
%Then $p\in C_1$ outputs a vector that does not contain the input value of any process in $C_2$, since it could not have received any of their inputs.

\paragraph{Scenario~3.} No process is faulty, but all messages out of $C_1$ and $C_2$ to other sets are arbitrarily delayed and all other messages arrive immediately. This scenario is indistinguishable to processes in $Q$ from both of the other scenarios. Furthermore, it is indistinguishable to $C_1$ from Scenario~2, and indistinguishable to $C_2$ from Scenario~1.
%Therefore, by the end of the round, $C_1$ receives the same messages as it does in Scenario~2, and $C_2$ receives the same messages as in Scenario~1.
Therefore, any pair of processes $p \in C_1$ and $p' \in C_2$ does not receive each other's message in this round despite both being correct and sending messages. This contradicts the unidirectionality property.
\end{proof}



\begin{claim}
Reliable broadcast can implement unidirectionality in a system with $f=1$ and $n\geq 3$.
\end{claim}
\begin{proof}
Consider the following protocol for creating a unidirectional round.

\begin{lstlisting}
Protocol for process p with input v:
    Phase 1: send (v,@$\sigma_p$@) to all //where @$\sigma_p$@ is $p$'s unforgeable signature for @$v$@
      wait to receive phase 1 messages with valid signatures from n-1 distinct processes
    Phase 2: forward all messages received to all
      wait to receive phase 2 messages from n-1 distinct processes, 
      such that each message is of the from [(@$v_1$@, @$\sigma_1$@), ... (@$v_m$@, @$\sigma_m$@)]  
        where m @$\geq$@ 2 and all signatures are valid and from distinct processes.
\end{lstlisting}

We claim that at the end of phase~2 of a \correct{} process $p$, the unidirectional property holds for $p$ with every other \correct{} process $p'$ for the input values.

%Note that if there is a fault and $n=2$, the unidirectional property vacuously holds.

Consider two correct processes $p$ and $p'$ executing the above protocol in a system with reliable broadcast, and let $Q$ be  the set containing the rest of the processes in the system. If $p$ receives $p'$'s message (or vice versa) directly in either phase, then the unidirectional property already holds. 

Thus, assume that neither $p$ nor $p'$ receives the other's message directly in either phase.
Note that all processes in $Q$ must receive at least one of $p$ or $p'$'s messages in phase~1, without loss of generality assume they receive $p$'s value. Furthermore, both $p$ and $p'$ receive all of $Q$'s phase~2 messages. Since valid phase~2 messages must contain $n-1$ values from phase~1 and are unforgeable, $Q$'s phase~2  message must contain $p$'s phase~1 message, which $p'$ now receives.
%
%Recall that $p$ waits to receive messages from $n-1 = n-f$ processes in phase~2, and that each of these messages must contain the phase~1 messages of at least $n-1$ distinct processes. If $p$ received a phase~2 message from $p'$, we are done. Thus, assume $p$ received phase~2 messages from all processes in $Q$, but not from $p'$. Furthermore, if any process $q\in Q$ reported $p'$'s message to $p$ in phase~2, unidirectionality again holds. Assume therefore that no process $q\in Q$ reported $p'$'s phase~1 value. This means that all $q\in Q$ received $p$'s message in phase~1, since they must have received $n-1$ messages. Thus, $q$ must report $p$'s phase~1 message to $p'$ in phase~2.
\end{proof}

\begin{conjecture}
Unidirectional communication can solve non-equivocating broadcast for $n \geq f + 1$. \kartik{to be moved}
\end{conjecture}
\begin{proof}
Consider the following algorithm, where a process $p$ can unforgeably sign a message $m$, denoted $m,p$:
\begin{lstlisting}
Algorithm for sender s with input v:
    send v,s to all
Algorithm for process p:
    upon receipt of msg = (v, s)
    send v,s to all
    wait until end of round
    if, for some p', received (v', s) from p' where v@$\neq$@v' @\label{line:checkMsgs}@
        commit @$\bot$@ @\label{line:commitbot}@
    else, commit v
\end{lstlisting}
We now show that if each round provides unidirectional communication, then the above algorithm solves non-equivocating broadcast for $n\geq f+1$, as long as a round always terminates in a system that tolerates $f$ faults.

\textbf{Agreement.} Assume some correct process $p$ commits $v\neq \bot$, and another correct process $q$ commits $v'$. For $p$ to commit $v$, it must have seen only messages with value $v$ by the end of its round. If $p$ received $q$'s message in its round, then $q$ must have sent $v$. Otherwise, by the unidirectionality of the round, $q$ must receive $p$'s message with value $v$ before the end of $q$'s round. In either case, $q$ saw the value $v$. Thus, it can either commit $v$ or commit $\bot$, but cannot commit any other value.

\textbf{Termination.} As long as the round is always finite, there is no other blocking call or loop in the algorithm, so it will terminate.

\textbf{Validity.} If the sender is correct, then it only ever signs one message. Thus, no other process can receive any other message with $s$'s signature, and therefore no correct process can commit on line~\ref{line:commitbot}.
\end{proof}

\begin{claim}
Zero-directionality cannot solve non-equivocating broadcast for $n \leq 3f$. \kartik{to be removed}
\end{claim}
\begin{proof}[Rough Sketch/Intuition]
We know that asynchronous message passing systems cannot prevent equivocation (even weak non-equivocation, which is achieved by this broadcast primitive, is not possible).\kartik{cite} We know this because we know that weak non-equivocation raises the fault tolerance of weak validity agreement from $3f+1$ to $2f+1$, but this is not possible in asynchronous message passing. \Naama{No longer sure of this, since non-equivocating broadcast is not enough for using in Clement's construction.}
\end{proof}

\begin{claim}
Non-equivocation (reliable broadcast) can solve weak Byzantine agreement with $n\geq 2f+1$. \kartik{move to section 2}
\end{claim}

\begin{proof}[Proof sketch.]
Known from Clement et al. and other papers~\cite{clement2012limited,chun2007attested}. But we need to cast them as reliable broadcast if that's the definition we're going for.
\end{proof}

\begin{claim}
Unidirectional communication can solve very weak Byzantine agreement with $n>f$.
\end{claim}

\begin{proof}
We show the result by showing a protocol for achieving very weak Byzantine agreement using unidirectional communication.
\begin{lstlisting}
Algorithm for process p with input v:
    send v to all processes
    wait until end of round
    if any received value v' @$\neq$@ v, 
        commit @$\bot$@
    else 
        commit v
\end{lstlisting}
\paragraph{Agreement.} Consider the set of values $V_i$ that a correct process $p_i$ receives by the end of its round, including its own input value $v_i$. If $|V_i| \geq 2$, then $p_i$ commits $\bot$. Thus, $p_i$ satisfies very weak agreement with every correct process $p_j$. Otherwise $|V_i| = 1$. Consider any other correct process $p_j$. Since the rounds are unidirectional and all correct processes send messages, either $p_i$ receives $p_j$'s input or vice versa. In either case, $p_j$ receives the message $v_i$, i.e., $v_i\in V_j$ (either from itself or from $p_i$). 
Therefore, by the protocol, $p_j$ cannot commit any value $v'$ such that $v' \neq v_i$ and $v' \neq \bot$.

\paragraph{Validity.} If all processes are correct and all started with the same input $v$, then for each process, all received values must be $v$. Therefore, all processes commit $v$, as required.
\end{proof}

\begin{claim}
Reliable broadcast cannot solve very weak Byzantine agreement with $n\leq 2f$.
\end{claim}

\begin{proof}
The proof of this claim follow from the classic partitioning argument.
Suppose the network is partitioned into two sets $P$ and $Q$ of size $\lfloor n/2 \rfloor$ and  $\lceil n/2 \rceil$ respectively. We show the result by a sequence of five worlds:
\paragraph{World~1.} Processes in $P$ are correct and start with input $0$ and processes in $Q$ crash. By the agreement and termination property of very weak Byzantine Agreement, all processes in $P$ commit $0$ or~$\bot$.

\paragraph{World~2.} Processes in $P$ and $Q$ start with input $0$. All messages within $P$ and within $Q$ arrive immediately, but any message between processes in $P$ and processes in $Q$ are arbitrarily delayed.  Then this world is indistinguishable to $P$ from World~1, and therefore processes in $P$ must terminate without receiving any messages from $Q$. However, due to the validity property, all processes in $P$ must commit~$0$.

\paragraph{World~3.} (Symmetric to World~1) Processes in $P$ crash, and processes in $Q$ start with input $1$. By the agreement and termination property of very weak Byzantine Agreement, all processes in $Q$ commit $1$ or~$\bot$.

\paragraph{World~4.} (Symmetric to World~2) Processes in $P$ and $Q$ start with input $1$. All messages within $P$ and within $Q$ arrive immediately, but any message between processes in $P$ and processes in $Q$ are arbitrarily delayed.  Then this world is indistinguishable to $P$ from World~3, and therefore processes in $P$ must terminate without receiving any messages from $Q$. However, due to the validity property, all processes in $P$ must commit~$1$.

\paragraph{World~5.} Processes in $P$ start with input $0$, processes in $Q$ start with input $1$, and all messages between $P$ and $Q$ are arbitrarily delayed. This world is indistinguishable to $P$ from World~2, and therefore all processes in $P$ commit $0$. Furthermore, it is indistinguishable to $Q$ from World~4, and therefore processes in $Q$ commit~$1$. This violates the agreement property.
\end{proof}

\begin{claim}
Unidirectional communication cannot implement reliable broadcast with $n\leq 2f$.
\end{claim}

\begin{proof}

\end{proof}

\begin{claim}
Unidirectionality can solve reliable broadcast with $n\geq 2f+1$.
\end{claim}


\subsection{Other questions and comments...}
\Naama{Could also discuss requiring certain levels of communication in the case where the sender is honest (or some other `good' case) vs the worst case.}

\Naama{Note also that we should be specifying the fault tolerance in all of the conjectures, since we know the amount of communication required changes with the fault tolerance.}



\begin{question}
How many bidirectional/unidirectional rounds are required to solve BB when the sender is honest? What about in general? How does the answer change as fault tolerance changes?
\Naama{For the general question (when the sender isn't necessarily honest, does Dolev-Strong imply $f+1$ bidirectional rounds?}
\end{question}







==> trinc.tex <==
\section{Implementing TrInc using SRB}\label{sec:trincInterface}

\begin{theorem}
Sequenced Reliable Broadcast can implement the interface specified in Algorithm~\ref{alg:hw-interface}.
\end{theorem}

\begin{proof}
   We present an implementation of the TrInc functionality using sequenced reliable broadcast. 
 
    \begin{lstlisting}
for each process p, 
initialize: k = 0, for each process q, C[q] = 0

attestation Attest(seq-num c, message m) {
    Broadcast(k, (c,m)); // k is the broadcast sequence number
    return (k, (c,m));}

bool CheckAttestation(attestation a, id q){
    upon delivering a message (k, c, m) from q
        if C[q] < c { @\label{line:checkseq}@
            store (k, (c,m));
            C[q] = c;   }
    if (I've stored a message (k,(c,m)) == a from q) {
        return true; }
    else{
        return false;}  }
    \end{lstlisting}
    
We now show that the above implementation satisfies the properties of the TrInc interface. In particular, we show that (1) $CheckAttestation(a,q)$ would eventually return true if process $q$ correctly invoked a $T_q$.Attest instance that returned $a$, and (2) $CheckAttestation(a,q)$ returns false if $a$ was not correctly attested by $T_q$.

%For the first property, note that $k$ and $c$ are initialized to the same value. Furthermore, if $c$ is larger than $k$, a non-null value is returned, and $k$ is updated to $c$. Otherwise, null is returned, and $k$ is not updated. The rest of the proof follows by a simple induction.

For the first property, recall that by property~\ref{prop:SRBweak-termination}, if $q$ correctly invoked broadcast for value $(k,c,m)$, then eventually every correct process will deliver $(k,c,m)$ from $q$. Furthermore, $T_q$.Attest(c,m) will return $(k,c,m)$ in this case.  Therefore, eventually, some invocation of $CheckAttestation(a,q)$ by each correct process $p$ will happen after the process already delivered $(k,c,m)$. Recall that a correct attestation always uses a sequence number $c$ that is larger than all previous ones. Therefore, if $q$ correctly attested its message delivered by $p$, the check on Line~\ref{line:checkseq} passes, and $p$ stores this message. So the $CheckAttestation(a,q)$ call by $p$ will return true.

Secondly, by property~\ref{prop:SRBintegrity} of SRB, if a correct process $p$ delivered an attestation $a$ from $q$, $q$ must have broadcast it. Therefore, by definition, there was an Attest by $q$ that returned $a$. A $CheckAttestation(a,q)$ by $p$ returns false if $p$ did not deliver $a$ from $q$. 
\end{proof}

==> uni-srb-algo.tex <==
\section{Sequenced Reliable Broadcast from Unidirectionality}\label{sec:uni-srb}


\renewcommand{\figurename}{Algorithm}
\begin{figure}
	\caption{Sequenced Reliable Broadcast using Unidirectional Rounds}
	\begin{lstlisting}[columns=fullflexible,breaklines=true]
Code @\texttt{for}@ process p
	next_p; //next index to deliver from sender. Initially, next_p=1
	state; //@$\in$@{WaitForSender,WaitForL1Proof,WaitForL2Proof}. Initially, state=WaitForSender
	my_seq; //most recent sequence number used to broadcast a message, if p is the sender
	
	void broadcast (m){
	    my_seq += 1;
		send sign((my_seq,m)) to all; @\label{line:broadcastWrite}@   }
	
	bool maybeDeliver() {
	    k = next_p;
	    val = checkL2Proof(k);@\label{line:readL2proof}@
		if (val != null) {
			deliver(k, val, q);@\label{line:deliver}@
			next_p += 1;
			state = WaitForSender;
			return true;	}
	    return false;
	}
	
	void try_deliver(q) {
		if (state == WaitForSender) {
		    upon receiving message val=(j,m) from q
		        if (maybeDeliver(val)){return;}
			    if (!sValid(q, val) || j!=k) {	return;	}
			    Send sign(val) to all;@\label{line:copyVal}@
			    state = WaitForL1Proof; }
	
		if (state == WaitForL1Proof) {
			checkedVals = @$\emptyset$@;
			do {
			    upon receiving message v from process r @\label{line:readMessage}@
				    if (maybeDeliver(val)){return;}
				    if (validateValue(v,val,k,q)) {checkedVals.add((r,v));} 
			} until (unidirectional round is finshed and size(checkedVals) @$\geq$@ t+1)
	
			l1prf = sign(checkedVals);
			send l1prf to all;@\label{line:writel1prf}@
			state = WaitForL2Proof; }   }
	
		if (state == WaitForL2Proof){
			checkedL1Prfs = @$\emptyset$@;
			do{
			    upon receiving message prf from r @\label{line:readL1proof}@
				    if (maybeDeliver(val)){return;}
				    if (validateL1Prf(prf,val,k,q)) {checkedL1Prfs.add((r,prf));}
			} until (unidirectional round finished and size(checkedL1Prfs) @$\geq$@ t+1)
	
		l2prf = sign(checkedL1Prfs);
		send l2prf to all; }   } }@\label{line:writeL2proof1}@
	\end{lstlisting}
\label{alg:uni-srb}
\end{figure}

\begin{figure}
	\caption{Helper functions for Sequenced Reliable Broadcast algorithm}
\begin{lstlisting}[firstnumber=52]
value checkL2proof(proof,k) {
    if proof contains at least one sequence number and at least one value{
        j = first sequence number in proof;
        if (j@$\neq$@k) {return null;}@\label{line:seqnum}@
		val = first value in proof;
		if (validateL2Prf(proof,val,k,p)) {
			Send proof to all; @\label{line:writeL2proof2}@
			return val; }   }   }
	return null;    }
	
bool validateValue(v, val, k, q){
	if (v == val && sValid(q,v) && key == k){
		return true; }
	return false;	}
	
bool validateL1Prf(proof, val, k, q){
	if (size(proof) @$\geq$@ t+1) {
		for each (i,(v, s)) in proof {
			if (!validateValue(v,val,k,q) || !sValid(i, (v,s)){
				return false;	} 	}	}
	return true;	}

bool validateL1Prf(proof, val, k, q){
	if (size(proof) @$\geq$@ t+1 && @$\forall$@ 
		for each (i,(l1prf,s)) in proof {
			if (!validateL1Proof(l1prf,val,k,q) || !sValid(i, (l1prf, s))){
				return false;}	} 	}
	return true;	}
\end{lstlisting}
\label{alg:uni-srb-help}
\end{figure}
%\Naama{Check validation pseudocode.}

We now prove the following key lemma:

\begin{lemma}\label{lem:SMnon-eq}
	Sequenced Reliable Broadcast can be solved using unidirectional communication with $n\geq 2t+1$ processes.
\end{lemma}

We prove the lemma by showing that Algorithm~\ref{alg:uni-srb} correctly implements sequenced reliable broadcast. 
We do so by showing that the algorithm satisfies each of the required properties.

\begin{lemma}\label{lem:deliverseq}
If some \correct{} process $q$ delivers a message with sequence number $k$ from $p$ at time $t$, then $q$ delivered messages with all sequence numbers $1\leq k' < k$ before time $t$.
\end{lemma}
\begin{proof}
Processes deliver a message $(k,m)$ on Line~\ref{line:deliver}, which is only executed if checkL2Proof(p,k) returns a non-null value, which a correct process calls with $k$ equal to the next sequence number to be delivered from the sender. This sequence number starts at $1$ and is only ever incremented upon delivery of a value from $p$. Note that by Line~\ref{line:seqnum} in checkL2Proof(), checkL2Proof returns null if the sequence number does not match. The rest of the proof can be completed by a straightforward induction.
\end{proof}
	
\begin{lemma}
If the sender $p$ is correct, then every correct process eventually delivers every message that $p$ broadcasts.
\end{lemma}

\begin{proof}
Let $p$ be a correct sender. We assume by contradiction that there exists some message $(k,m)$ the $p$ broadcasts, but that some correct process $q$ never delivers. Furthermore, assume without loss of generality that $k$ is the smallest sequence number for which $p$ broadcasts a message that some correct process never delivers. That is, all correct processes must eventually deliver all messages $(k',m')$ from $p$, for $k' < k$. Thus, all correct processes must eventually increment $last[p]$ to $k$.

We consider two cases, depending on whether or not some process eventually sends an L2 proof for some $(k,m')$ message from $p$.

First consider the case where no process ever sends an L2 proof of any value $(k,m')$ from $p$.
Since $p$ is correct, upon broadcasting $(k,m)$, $p$ must send a signed copy of $(k,m)$ (line~\ref{line:broadcastWrite}). Since $p$ is correct, it sends $(k,m)$ to all processes, and never sends any other message with that sequence number to any process. So, every correct process will eventually receive  $(k,m)$ in line~\ref{line:readMessage}, sign and send it to all others, and change their state to WaitForL1Proof. 
%\Naama{What about processes that terminate before that because they see an L2Proof?}

Furthermore, since $p$ is correct and we assume signatures are unforgeable, no process $q$ can send any other valid value $(k',m')\neq(k,m)$ to any correct process $r$ and have that value validated by $r$. Thus, eventually each correct process will add at least $t+1$ copies of $(k,m)$ to its checkedVals, sign and send an L1proof consisting of these values, and change their state to WaitForL2Proof. 

Therefore, all correct processes will eventually receive at least $t+1$ valid L1 Proofs for $(k,m)$ in line~\ref{line:readL1proof} and construct and send valid L2 proofs for $(k,m)$. This contradicts the assumption that no L2 proof is ever sent. 

In the case where there is some L2 proof, by the argument above, the only value it can prove is $(k,m)$. 
Therefore, all correct processes will receive at least one valid L2 proof and deliver. This contradicts our assumption that $q$ is correct but does not deliver $(k,m)$ from $p$.
\end{proof}
	
\begin{lemma}
If some correct process $q$ delivers message $m$ with sequence number $k$ from $p$, then eventually every correct process delivers $m$ with sequence number $k$ from $p$.
\end{lemma}
\begin{proof}
Let $q$ be a correct process that delivers $(k,m)$, and let $q'$ be another correct process. Assume by contradiction that $q'$ never delivers $(k,m)$ from $p$. 

We consider two cases.

\textsc{Case 1.} $q'$ eventually delivers some other message $(k,m')$ from $p$, where $m\neq m'$.

Since $q$ and $q'$ are correct, they must have received valid L2 proofs at line~\ref{line:readL2proof} before delivering $(k,m)$ and $(k,m')$ respectively. Let $\mathcal{Q}$ and $\mathcal{Q'}$ be those valid proofs for $(k,m)$ and $(k,m')$ respectively. $\mathcal{Q}$ (resp. $\mathcal{Q'}$) consists of at least $t+1$ valid L1 proofs; therefore, at least one of those proofs was created by some correct process $r$ (resp. $r'$). Since $r$ (resp. $r'$) is correct, it must have sent $(k,m)$ (resp. $(k,m')$) to all processes in line~\ref{line:copyVal}. Recall that both $r$ and $r'$ communicate through unidirectional rounds, and wait until their round ends before compiling and sending their L1Proofs. Since both $r$ and $r'$ are correct, at least one of them must have received the other's message before compiling its L1 proof.
%
Assume without loss of generality that $r'$ received $r$'s message. Since $r'$ is correct, it cannot have then compiled an L1 proof for $(k,m')$. We have reached a contradiction.

\textsc{Case 2.} $q'$ never delivers any message from $p$ with sequence number $k$.

By Lemma~\ref{lem:deliverseq}, if $q$ delivers $(k,m)$ from $p$, then for all $i<k$ there exists $m_i$ such that $q$ delivered $(i,m_i)$ from $p$ before delivering $(k,m)$.

Assume without loss of generality that $k$ is the smallest key for which $q'$ does not deliver any message from $p$. Thus, $q'$ must have delivered $(i,m_i')$ from $p$ for all $i<k$; thus, $q'$ must have incremented $last[p]$ to $k$. Since $q'$ never delivers any message from $p$ for sequence number $k$, $q'$'s $last[p]$ will never increase past $k$.

Since $q$ delivers $(k,m)$ from $p$, then $q$  must have sent a valid L2 proof $\mathcal{P}$ of $(k,m)$ in line~\ref{line:writeL2proof1} or~\ref{line:writeL2proof2}. Thus, $q'$ will eventually receive this message. Since $q'$'s $last[p]$ eventually reaches $k$ and never increases past $k$, $q'$ will eventually call checkL2Proof with sequence number $k$, and checkL2Proof will eventually return a non-null value, causing $q'$ to deliver a value for sequence number $k$. We have reached a contradiction.
\end{proof}

	
\begin{lemma}
If some \correct{} process delivers a message $m$ from $p$, then $p$ broadcast $m$ at some earlier point in time.
\end{lemma}

\begin{proof}
We show that if a correct process $q$ delivers $(k,m)$ from a correct sender $p$, then $p$ broadcast $(k,m)$.
Correct processes only deliver values for which a valid L2 proof exists (lines~\ref{line:readL2proof}---\ref{line:deliver}). Therefore, $q$ must have received a valid L2 proof $\mathcal{Q}$ for $(k,m)$. $\mathcal{Q}$ consists of at least $t+1$ L1 proofs for $(k,m)$ and each L1 proof consists of at least $t+1$ matching copies of $(k,m)$, signed by $p$. Since $p$ is correct and we assume signatures are unforgeable, $p$ must have broadcast $(k,m)$ (otherwise $p$ would not have attached its signature to $(k,m)$). 
\end{proof}

